Trio-ViT: Post-Training Quantization and Acceleration for Softmax-Free Efficient Vision Transformer

Motivated by the huge success of Transformers in the field of natural language processing (NLP), Vision Transformers (ViTs) have been rapidly developed and achieved remarkable performance in various computer vision tasks. However, their huge model sizes and intensive computations hinder ViTs' deployment on embedded devices, calling for effective model compression methods, such as quantization. Unfortunately, due to the existence of hardware-unfriendly and quantization-sensitive non-linear operations, particularly {Softmax}, it is non-trivial to completely quantize all operations in ViTs, yielding either significant accuracy drops or non-negligible hardware costs. In response to challenges associated with \textit{standard ViTs}, we focus our attention towards the quantization and acceleration for \textit{efficient ViTs}, which not only eliminate the troublesome Softmax but also integrate linear attention with low computational complexity, and propose Trio-ViT accordingly. Specifically, at the algorithm level, we develop a {tailored post-training quantization engine} taking the unique activation distributions of Softmax-free efficient ViTs into full consideration, aiming to boost quantization accuracy. Furthermore, at the hardware level, we build an accelerator dedicated to the specific Convolution-Transformer hybrid architecture of efficient ViTs, thereby enhancing hardware efficiency. Extensive experimental results consistently prove the effectiveness of our Trio-ViT framework. {Particularly, we can gain up to $\uparrow$$\mathbf{3.6}\times$, $\uparrow$$\mathbf{5.0}\times$, and $\uparrow$$\mathbf{7.3}\times$ FPS under comparable accuracy over state-of-the-art ViT accelerators, as well as $\uparrow$$\mathbf{6.0}\times$, $\uparrow$$\mathbf{1.5}\times$, and $\uparrow$$\mathbf{2.1}\times$ DSP efficiency.} Codes are available at \url{https://github.com/shihuihong214/Trio-ViT}.

==> section/Abstract.tex <==
\begin{abstract}
% 	Multiplication is arguably the most cost-dominant operation in modern deep neural networks (DNNs), limiting their achievable efficiency and thus more extensive deployment into resource-constrained applications. To tackle this limitation, pioneering works have developed handcrafted multiplication-less DNNs, which require expert knowledge and time-consuming manual iteration, calling for fast development tools. To this end, we propose NASA (neural architecture search and acceleration framework), which enables automated multiplication-less DNN development and integrates dedicated multiplication-less accelerators for boosted DNN efficiency. Specifically, NASA adopts a neural architecture search (NAS) space that augments state-of-the-art ones with hardware inspired multiplication-less operators, such as shift and add, and a differentiable NAS search algorithm to automatically search for multiplication-less DNNs; On top of that, NASA further develops a dedicated accelerator for the NASA-NAS resulting DNNs to better leverage their algorithmic properties for boosting hardware efficiency. Experimental results and ablation studies validate the advantages of our proposed NASA algorithm-hardware co-design framework in terms of achieved accuracy and efficiency. All the codes will be released publicly upon acceptance.

Multiplication is arguably the most cost-dominant operation in deep neural networks (DNNs), limiting their achievable efficiency and thus more extensive applications into resource-constrained devices. As such, pioneering works have developed handcrafted multiplication-less DNNs, which require expert knowledge and time-consuming manual iteration, calling for fast development tools. To this end, we propose NASA (a Neural Architecture Search and Acceleration framework), which enables automated hybrid DNN development and integrates dedicated accelerators to better leverage hybrid DNNs’ algorithmic properties for boosted hardware efficiency. Extensive experiments validate the advantages of our proposed NASA algorithm-hardware co-design framework in terms of achieved accuracy and efficiency. 
\end{abstract}


